Adaptive Discounting of Implicit Language Models in RNN-Transducers

RNN-Transducer (RNN-T) models have become synonymous with streaming end-to-end ASR systems. While they perform competitively on a number of evaluation categories, rare words pose a serious challenge to RNN-T models. One main reason for the degradation in performance on rare words is that the language model (LM) internal to RNN-Ts can become overconfident and lead to hallucinated predictions that are acoustically inconsistent with the underlying speech. To address this issue, we propose a lightweight adaptive LM discounting technique AdaptLMD, that can be used with any RNN-T architecture without requiring any external resources or additional parameters. AdaptLMD uses a two-pronged approach: 1) Randomly mask the prediction network output to encourage the RNN-T to not be overly reliant on it's outputs. 2) Dynamically choose when to discount the implicit LM (ILM) based on rarity of recently predicted tokens and divergence between ILM and implicit acoustic model (IAM) scores. Comparing AdaptLMD to a competitive RNN-T baseline, we obtain up to 4% and 14% relative reductions in overall WER and rare word PER, respectively, on a conversational, code-mixed Hindi-English ASR task.

==> final_tables/table1.1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\scalebox{0.57}{
\begin{tabular}{|l|l|l|r|r|r|r|r|}
\hline
Train Data
(Hours)&
  Test  Data &
  ASR System &
  \multicolumn{1}{l|}{WER} &
  \multicolumn{1}{l|}{CER} &
  \multicolumn{1}{l|}{PER} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Rare-\\ PER\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Rare-\\ CER\end{tabular}} \\ \hline \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ALL\\ (477.25 hrs)\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ALL\\ (x hrs)\end{tabular}} &
  RNNT &
  14.50 &
  13.50 &
  12.00 &
  57.56 &
  71.19 \\ \cline{3-8} 
 &
   &
  ILMT &
  14.50 &
  13.40 &
  12.10 &
  53.81 &
  66.63 \\ \cline{3-8} 
 &
   &
 \sysname &
  \textbf{14.10} &
  \textbf{13.10} &
  \textbf{11.80} &
  \textbf{52.23} &
  \textbf{63.86} \\ \hline \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} Telco (102.83) + Retail(96.13)\\ Insurance(128.32) Total (327.28) hrs\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Test \\ x hrs\end{tabular}} &
  RNN\_T &
  14.50 &
  13.60 &
  12.30 &
  66.93 &
  68.23 \\ \cline{3-8} 
 &
   &
  ILMT &
  14.60 &
  13.40 &
  12.00 &
  69.32&
  70.50 \\ \cline{3-8} 
 &
   &
 \sysname &
  \textbf{14.20} &
  \textbf{13.10} &
  \textbf{11.90} &
  \textbf{63.15} &
  \textbf{59.60} \\ \hline \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Banking(149.97) + Retail(96.13) \\ +Insurance (128.32) Total(374.42 hrs)\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Test \\ x hrs\end{tabular}} &
  RNN\_T &
  15.20 &
  14.00 &
  12.70 &
   67.98 &
 76.69 \\ \cline{3-8} 
 &
  &
  ILMT & 15.90&	14.50	& \textbf{12.30} &63.83&	74.20
%   ILMT &
%   19.2 &
%   18.3 &
%   16.6 &
%   63.83 &
%   70.20 
\\ \cline{3-8} 
 &
   &
 \sysname &
  \textbf{14.90} &
  \textbf{13.60} &
  \textbf{12.30} &
  \textbf{60.20} &
  \textbf{63.29} \\ \hline \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Banking(149.97) + Telco (102.83) \\ +Insurance (128.32) Total (381.12) hrs\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Test\\ z hrs\end{tabular}} &
  RNN\_T &
  14.20 &
  13.20 &
  12.00 & 
  65.32&
  72.73 \\ \cline{3-8} 
 &
   &
  ILMT &
  14.10 &
  13.80 &
  11.80 &
64.65 &
  65.73 \\ \cline{3-8} 
 &
   &
 \sysname &
  \textbf{13.80} &
  \textbf{12.90} &
  \textbf{11.60} &
  \textbf{63.10} &
  \textbf{63.83} \\ \hline \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Banking(149.97) + Telco (102.83) \\ +Retail (96.13) Total (348.93) hrs\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Test \\ y hrs\end{tabular}} &
  RNN\_T &
  15.00 &
  14.40 &
  13.10 &
  66.93 &
  68.23 \\ \cline{3-8} 
 &
   &
  ILMT &
  15.90 &
  14.50 &
  13.20 &
69.33&
 70.52 \\ \cline{3-8} 
 &
   &
  \sysname &
  \textbf{15.10} &
  \textbf{14.00} &
  \textbf{12.70} &
  \textbf{63.51} &
  \textbf{59.60} \\ \hline 
\end{tabular}
}
\caption{ASR Performance trained and tested on in-domain data }
\label{tab:indomain}
\end{table}

==> rnnt_image.tex <==
\begin{tikzpicture}[
mybox/.style={minimum width=4cm,draw,thick,align=center,minimum height=1.8cm},
arrow/.style = {thick,-stealth}
]


%nodes
\node[mybox,fill=blue!40!white, label=above:$g_u$] (LM) {Prediction Network};
\node[right=1cm of LM, mybox,fill=red!40!white,label=above:{$\mathbf{h}=\{ h_1, h_2, h_3, ... h_T \}$}] (AM) {Transcription Network};
\node[yshift=4.5cm, right=-1.5cm of LM, mybox,fill=green!40!white, label=above:{$P(y_{t,u} | \vy_{<u}, x_t)$}] (softmax) {Joint Softmax};
\node[circle, below = of softmax, yshift=0.25 cm, label=below:{$(h_t \oplus g_u)$},fill=purple!40!yellow, scale=1,path picture={
\draw[black] (path picture bounding box.west) -- (path picture bounding box.east);
\draw[black] (path picture bounding box.north) -- (path picture bounding box.south);
}] (jointop) {};
\node [below = of AM] (input-x){$\mathbf{x} = \{x_1, x_2, x_3 ... x_T\}$};
\node [below = of LM] (input-y){$y_{u-1}$};

%arrows
\draw [arrow] (input-y) -- (LM);
\draw [arrow] (input-x) -- (AM);
\draw [arrow] (LM.north)+(0,0.5cm) |- (jointop);
\draw [arrow] (AM.north)+(0,0.5cm) |- (jointop);
\draw [arrow] (jointop.north) -- (softmax);
\draw [dashed] (input-y.east)+(-2cm,0) -- (input-y.west);
%\draw [line] (jointop.north) -- (jointop.south);
%\draw [line] (jointop.east) -- (jointop.west);
%\fill[blue!40!white] (0,0) rectangle (4,2);
%\fill[red!40!black] (5,0) rectangle (9,2);
\end{tikzpicture} 


==> table-outdomain.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\scalebox{0.6}{
%\begin{tabular}{p{0.35\linewidth} | p{0.6\linewidth}}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
 &
  Split &
  Method &
  WER &
  CER &
  PER &
  R-PER-all &
  R-CER-all &
  Ent-PER-all &
  Ent-CER-all &
  Ent-WER\_OD &
  Ent-WER\_OD\_En &
  R-WER\_OD &
  R-WER\_OD\_En \\ \hline
\multirow{6}{*}{BANKING} &
  \multirow{3}{*}{Val} &
  RNN-T &
  21.20 &
  19.20 &
  16.20 &
  71.80 &
  76.24 &
  21.39 &
  22.52 &
  33.20 &
  35.20 &
  98.60 &
  99.80 \\ \cline{3-14} 
 &
   &
  ILMT &
  21.30 &
  18.80 &
  17.10 &
  66.14 &
  \textbf{70.67} &
  21.54 &
  23.00 &
  33.20 &
  34.50 &
  97.50 &
  100.00 \\ \cline{3-14} 
 &
   &
  \textbf{AdaptLMD} &
  \textbf{20.50} &
  \textbf{18.00} &
  \textbf{16.30} &
  \textbf{67.13} &
  71.95 &
  \textbf{20.40} &
  \textbf{21.40} &
  \textbf{31.50} &
  \textbf{37.00} &
  \textbf{99.60} &
  \textbf{99.00} \\ \cline{2-14} 
 &
  \multirow{3}{*}{Test} &
  RNN-T &
  22.40 &
  20.00 &
  18.50 &
  70.88 &
  75.95 &
  24.53 &
  25.85 &
  37.70 &
  40.40 &
  100.40 &
  100.20 \\ \cline{3-14} 
 &
   &
  ILMT &
  \textbf{22.40} &
  19.50 &
  17.90 &
  67.14 &
  71.05 &
  24.58 &
  26.51 &
  38.60 &
  40.60 &
  99.60 &
  100.00 \\ \cline{3-14} 
 &
   &
  \textbf{AdaptLMD} &
  \textbf{21.50} &
  \textbf{18.70} &
  \textbf{17.10} &
  \textbf{67.44} &
  \textbf{71.77} &
  \textbf{22.34} &
  \textbf{23.44} &
  \textbf{37.00} &
  \textbf{38.70} &
  \textbf{99.10} &
  \textbf{100.40} \\ \hline
\multirow{6}{*}{INSURANCE} &
  \multirow{3}{*}{Val} &
  RNN-T &
  18.70 &
  17.40 &
  15.90 &
  67.61 &
  73.90 &
  30.78 &
  34.23 &
  30.80 &
  60.30 &
  98.70 &
  100.30 \\ \cline{3-14} 
 &
   &
  ILMT &
  18.90 &
  17.40 &
  15.80 &
  63.78 &
  69.84 &
  28.46 &
  32.61 &
  30.70 &
  59.80 &
  98.40 &
  99.70 \\ \cline{3-14} 
 &
   &
  \textbf{AdaptLMD} &
  \textbf{17.80} &
  \textbf{16.10} &
  \textbf{14.60} &
  \textbf{58.39} &
  \textbf{63.73} &
  \textbf{28.52} &
  \textbf{31.60} &
  \textbf{29.40} &
  \textbf{58.30} &
  \textbf{98.80} &
  \textbf{99.70} \\ \cline{2-14} 
 &
  \multirow{3}{*}{Test} &
  RNN-T &
  18.40 &
  17.70 &
  16.10 &
  70.17 &
  76.68 &
  41.56 &
  45.25 &
  53.70 &
  38.30 &
  98.40 &
  99.80 \\ \cline{3-14} 
 &
   &
  ILMT &
  18.70 &
  17.60 &
  15.90 &
  65.75 &
  72.20 &
  37.85 &
  42.28 &
  54.30 &
  39.40 &
  97.80 &
  100.80 \\ \cline{3-14} 
 &
   &
  \textbf{AdaptLMD} &
  \textbf{17.70} &
  \textbf{16.40} &
  \textbf{14.80} &
  \textbf{60.69} &
  \textbf{67.20} &
  \textbf{36.04} &
  \textbf{40.14} &
  \textbf{50.40} &
  \textbf{36.70} &
  \textbf{97.50} &
  \textbf{100.60} \\ \hline
\multirow{6}{*}{RETAIL} &
  \multirow{3}{*}{Val} &
  RNN-T &
  23.70 &
  21.60 &
  19.80 &
  72.44 &
  78.24 &
  49.21 &
  50.79 &
  40.90 &
  79.20 &
  96.10 &
  100.20 \\ \cline{3-14} 
 &
   &
  ILMT &
  23.40 &
  20.80 &
  18.90 &
  68.07 &
  74.62 &
  44.18 &
  46.26 &
  43.40 &
  81.70 &
  98.00 &
  100.70 \\ \cline{3-14} 
 &
   &
  \textbf{AdaptLMD} &
  \textbf{22.70} &
  \textbf{20.30} &
  \textbf{18.50} &
  \textbf{68.55} &
  \textbf{74.99} &
  \textbf{47.50} &
  \textbf{50.12} &
  \textbf{42.10} &
  \textbf{79.20} &
  \textbf{96.60} &
  \textbf{100.50} \\ \cline{2-14} 
 &
  \multirow{3}{*}{Test} &
  RNN-T &
  24.70 &
  22.40 &
  20.60 &
  76.74 &
  81.29 &
  46.77 &
  45.77 &
  50.40 &
  74.20 &
  97.90 &
  100.20 \\ \cline{3-14} 
 &
   &
  ILMT &
  24.50 &
  21.40 &
  19.70 &
  72.41 &
  77.52 &
  39.11 &
  38.15 &
  55.50 &
  69.10 &
  97.90 &
  100.50 \\ \cline{3-14} 
 &
   &
  \textbf{AdaptLMD} &
  \textbf{23.70} &
  \textbf{21.20} &
  \textbf{19.50} &
  \textbf{72.18} &
  \textbf{78.35} &
  \textbf{45.41} &
  \textbf{43.70} &
  \textbf{50.00} &
  \textbf{68.30} &
  \textbf{96.70} &
  \textbf{100.50} \\ \hline
\multirow{6}{*}{TELCO} &
  \multirow{3}{*}{Val} &
  RNN-T &
  19.00 &
  18.80 &
  17.20 &
  72.07 &
  76.70 &
  17.43 &
  18.87 &
  19.90 &
  28.90 &
  99.30 &
  100.00 \\ \cline{3-14} 
 &
   &
  ILMT &
  19.20 &
  18.30 &
  16.60 &
  63.84 &
  70.21 &
  16.47 &
  18.32 &
  19.50 &
  24.40 &
  103.30 &
  100.50 \\ \cline{3-14} 
 &
   &
  \textbf{AdaptLMD} &
  \textbf{18.40} &
  \textbf{17.70} &
  \textbf{16.10} &
  \textbf{62.97} &
  \textbf{67.74} &
  \textbf{16.40} &
  \textbf{17.97} &
  \textbf{19.80} &
  \textbf{25.20} &
  \textbf{98.70} &
  \textbf{99.50} \\ \cline{2-14} 
 &
  \multirow{3}{*}{Test} &
  RNN-T &
  19.40 &
  18.60 &
  17.10 &
  68.27 &
  72.57 &
  30.17 &
  33.26 &
  19.90 &
  61.00 &
  98.00 &
  100.50 \\ \cline{3-14} 
 &
   &
  ILMT &
  19.30 &
  18.10 &
  16.40 &
  63.79 &
  68.97 &
  29.31 &
  33.23 &
  20.00 &
  57.70 &
  97.40 &
  100.20 \\ \cline{3-14} 
 &
   &
  \textbf{AdaptLMD} &
  \textbf{18.60} &
  \textbf{17.50} &
  \textbf{16.00} &
  \textbf{64.27} &
  \textbf{68.59} &
  \textbf{29.33} &
  \textbf{32.50} &
  \textbf{19.00} &
  \textbf{62.40} &
  \textbf{94.90} &
  \textbf{99.30} \\ \hline
\end{tabular}}
\caption{}
\label{tab:my-table}
\end{table*}

==> table-outdomain2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{FFFFFF} 
Test &
  Split &
  Method &
  WER &
  CER &
  PER &
  \begin{tabular}[c]{@{}c@{}}Rare\\ PER\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Rare\\ CER\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Entity\\ PER\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Entity\\ CER\end{tabular} &

  \begin{tabular}[c]{@{}c@{}}Entity\\ WER\\OD\_Hi\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Entity\\ WER\\OD\_En\end{tabular} \\ \hline
 &
   &
  RNN-T &
  21.20 &
  19.20 &
  16.20 &
  71.80 &
  76.24 &
  21.39 &
  22.52 &
  33.20 &
  35.20 \\ \cline{3-12} 
 &
   &
  ILMT &
  21.30 &
  18.80 &
  17.10 &
  66.14 &
  \textbf{70.67} &
  21.54 &
  23.00 &
  33.20 &
  34.50 \\ \cline{3-12} 
 &
  \multirow{-3}{*}{Val} &
  \textbf{\sysnmae} &
  \textbf{20.50} &
  \textbf{18.00} &
  \textbf{16.30} &
  \textbf{67.13} &
  71.95 &
  \textbf{20.40} &
  \textbf{21.40} &
  \textbf{31.50} &
  \textbf{37.00} \\ \cline{2-12} 
 &
   &
  RNN-T &
  22.40 &
  20.00 &
  18.50 &
  70.88 &
  75.95 &
  24.53 &
  25.85 &
  37.70 &
  40.40 \\ \cline{3-12} 
 &
   &
  ILMT &
  \textbf{22.40} &
  19.50 &
  17.90 &
  67.14 &
  71.05 &
  24.58 &
  26.51 &
  38.60 &
  40.60 \\ \cline{3-12} 
\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Test-\\ \\ BANKING\end{tabular}} &
  \multirow{-3}{*}{Test} &
  \textbf{\sysname} &
  \textbf{21.50} &
  \textbf{18.70} &
  \textbf{17.10} &
  \textbf{67.44} &
  \textbf{71.77} &
  \textbf{22.34} &
  \textbf{23.44} &
  \textbf{37.00} &
  \textbf{38.70} \\ \hline
 &
   &
  RNN-T &
  18.70 &
  17.40 &
  15.90 &
  67.61 &
  73.90 &
  30.78 &
  34.23 &
  30.80 &
  60.30 \\ \cline{3-12} 
 &
   &
  ILMT &
  18.90 &
  17.40 &
  15.80 &
  63.78 &
  69.84 &
  28.46 &
  32.61 &
  30.70 &
  59.80 \\ \cline{3-12} 
 &
  \multirow{-3}{*}{Val} &
  \textbf{\sysname} &
  \textbf{17.80} &
  \textbf{16.10} &
  \textbf{14.60} &
  \textbf{58.39} &
  \textbf{63.73} &
  \textbf{28.52} &
  \textbf{31.60} &
  \textbf{29.40} &
  \textbf{58.30} \\ \cline{2-12} 
 &
   &
  RNN-T &
  18.40 &
  17.70 &
  16.10 &
  70.17 &
  76.68 &
  41.56 &
  45.25 &
  53.70 &
  38.30 \\ \cline{3-12} 
 &
   &
  ILMT &
  18.70 &
  17.60 &
  15.90 &
  65.75 &
  72.20 &
  37.85 &
  42.28 &
  54.30 &
  39.40 \\ \cline{3-12} 
\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Test-\\ INSURANCE\end{tabular}} &
  \multirow{-3}{*}{Test} &
  \textbf{\sysname} &
  \textbf{17.70} &
  \textbf{16.40} &
  \textbf{14.80} &
  \textbf{60.69} &
  \textbf{67.20} &
  \textbf{36.04} &
  \textbf{40.14} &
  \textbf{50.40} &
  \textbf{36.70} \\ \hline
 &
   &
  RNN-T &
  23.70 &
  21.60 &
  19.80 &
  72.44 &
  78.24 &
  49.21 &
  50.79 &
  40.90 &
  79.20 \\ \cline{3-12} 
 &
   &
  ILMT &
  23.40 &
  20.80 &
  18.90 &
  68.07 &
  74.62 &
  44.18 &
  46.26 &
  43.40 &
  81.70 \\ \cline{3-12} 
 &
  \multirow{-3}{*}{Val} &
  \textbf{\sysname} &
  \textbf{22.70} &
  \textbf{20.30} &
  \textbf{18.50} &
  \textbf{68.55} &
  \textbf{74.99} &
  \textbf{47.50} &
  \textbf{50.12} &
  \textbf{42.10} &
  \textbf{79.20} \\ \cline{2-12} 
 &
   &
  RNN-T &
  24.70 &
  22.40 &
  20.60 &
  76.74 &
  81.29 &
  46.77 &
  45.77 &
  50.40 &
  74.20 \\ \cline{3-12} 
 &
   &
  ILMT &
  24.50 &
  21.40 &
  19.70 &
  72.41 &
  77.52 &
  \textbf{39.11} &
  \textbf{38.15} &
  55.50 &
  69.10 \\ \cline{3-12} 
\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Test-\\ RETAIL\end{tabular}} &
  \multirow{-3}{*}{Test} &
  \textbf{\sysname} &
  \textbf{23.70} &
  \textbf{21.20} &
  \textbf{19.50} &
  \textbf{72.18} &
  \textbf{78.35} &
  45.41 &
  43.70 &
  \textbf{50.00} &
  \textbf{68.30} \\ \hline
 &
   &
  RNN-T &
  19.00 &
  18.80 &
  17.20 &
  72.07 &
  76.70 &
  17.43 &
  18.87 &
  19.90 &
  28.90 \\ \cline{3-12} 
 &
   &
  ILMT &
  19.20 &
  18.30 &
  16.60 &
  63.84 &
  70.21 &
  16.47 &
  18.32 &
  19.50 &
  24.40 \\ \cline{3-12} 
 &
  \multirow{-3}{*}{Val} &
  \textbf{\sysname} &
  \textbf{18.40} &
  \textbf{17.70} &
  \textbf{16.10} &
  \textbf{62.97} &
  \textbf{67.74} &
  \textbf{16.40} &
  \textbf{17.97} &
  \textbf{19.80} &
  \textbf{25.20} \\ \cline{2-12} 
 &
   &
  RNN-T &
  19.40 &
  18.60 &
  17.10 &
  68.27 &
  72.57 &
  30.17 &
  33.26 &
  19.90 &
  61.00 \\ \cline{3-12} 
 &
   &
  ILMT &
  19.30 &
  18.10 &
  16.40 &
  63.79 &
  68.97 &
  29.31 &
  33.23 &
  20.00 &
  57.70 \\ \cline{3-12} 
\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Test-\\ TELCO\end{tabular}} &
  \multirow{-3}{*}{Test} &
  \textbf{\sysname} &
  \textbf{18.60} &
  \textbf{17.50} &
  \textbf{16.00} &
  \textbf{64.27} &
  \textbf{68.59} &
  \textbf{29.33} &
  \textbf{32.50} &
  \textbf{19.00} &
  \textbf{62.40} \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table*}

==> table1.1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\scalebox{0.6}{
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}r |
>{\columncolor[HTML]{FFFFFF}}r |
>{\columncolor[HTML]{FFFFFF}}r |
>{\columncolor[HTML]{FFFFFF}}r |
>{\columncolor[HTML]{FFFFFF}}r |
>{\columncolor[HTML]{FFFFFF}}r |
>{\columncolor[HTML]{FFFFFF}}r |
>{\columncolor[HTML]{FFFFFF}}r |
>{\columncolor[HTML]{FFFFFF}}r |}
\hline
\begin{tabular}[c]{@{}l@{}}Train \\ Data\end{tabular} &
  Split &
  EXP &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}WER} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}CER} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}PER} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Rare\\ PER\end{tabular}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Rare\\ CER\end{tabular}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Entity\\ PER\end{tabular}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Entity\\ CER\end{tabular}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Entity\\ WER\\ OD_Hi\end{tabular}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Entity\\ WER\\ OD_En\end{tabular}} \\ \hline
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  RNNT &
  14.5 &
  13.5 &
  12 &
  59.82 &
  71.19 &
  8.72 &
  8.97 &
  15.2 &
  17.4 \\ \cline{3-12} 
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  ILMT &
  14.5 &
  13.4 &
  12.1 &
  47.99 &
  63.63 &
  6.69 &
  8.71 &
  15.7 &
  17.4 \\ \cline{3-12} 
\cellcolor[HTML]{FFFFFF} &
  \multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}Test} &
  \sysname &
  14.1 &
  13.1 &
  11.8 &
  52.23 &
  69.32 &
  6.59 &
  8.26 &
  15.3 &
  17.9 \\ \cline{2-12} 
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  RNN-T &
  14 &
  13.3 &
  11.9 &
  57.55 &
  64.44 &
  7.39 &
  8.49 &
  18.1 &
  9.8 \\ \cline{3-12} 
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  ILMT &
  13.9 &
  13 &
  11.6 &
  53.80 &
  60.10 &
  6.97 &
  8.20 &
  18.2 &
  9.1 \\ \cline{3-12} 
\multirow{-6}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Banking+\\ Telco+\\ Retail+\\ Insurance\end{tabular}} &
  \multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}Val} &
  \sysname &
  13.6 &
  12.7 &
  11.4 &
  54.24 &
  60.86 &
  6.59 &
  7.92 &
  17.8 &
  8.5 \\ \hline
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  RNN\_T &
  14.2 &
  13.3 &
  12 &
  66.93 &
  68.23 &
  9.26 &
  9.92 &
  28.8 &
  7.3 \\ \cline{3-12} 
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF} &
  ILMT &
  14.2 &
  13.1 &
  11.8 &
  69.32 &
  70.58 &
  9.06 &
  9.16 &
  29.5 &
  6.8 \\ \cline{3-12} 
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Telco+\\ Retail+\\ Insurance\end{tabular}} &
  \multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Test\\ -Banking\end{tabular}} &
  \sysname &
  13.8 &
  12.8 &
  11.5 &
  63.51 &
  59.60 &
  7.09 &
  8.41 &
  28.3 &
  6.7 \\ \hline
\end{tabular}
}
\caption{}
\label{tab:my-table}
\end{table*}

==> table1.tex <==
% \usepackage{multirow}


\begin{table*}[h]
\refstepcounter{table}
\label{tab:my-table}
\scalebox{0.8}{
\begin{tabular}{|l|l|r|r|r|r|r|r|r|r|r|r|r|}
\hline
Exp. &
  Split &
  \multicolumn{1}{l|}{WER} &
  \multicolumn{1}{l|}{CER} &
  \multicolumn{1}{l|}{PER} &
  \multicolumn{1}{l|}{R-PER} &
  \multicolumn{1}{l|}{R-CER} &
  \multicolumn{1}{l|}{En-PER} &
  \multicolumn{1}{l|}{En-CER} &
  \multicolumn{1}{l|}{En-WER} &
  \multicolumn{1}{l|}{En-WER-eng} &
  \multicolumn{1}{l|}{R-WER} &
  \multicolumn{1}{l|}{R-WER\_eng} \\ \hline
\multirow{2}{*}{RNNT}                    & Test & 14.5 & 13.5 & 12   & 59.82 & 71.19 & 8.72 & 8.97 & 15.2 & 17.4 & 116.9 & 122.2 \\ \cline{2-13} 
                                         & Val  & 14   & 13.3 & 11.9 & 57.55 & 64.44 & 7.39 & 8.49 & 18.1 & 9.8  & 97.3  & 100.7 \\ \hline
\multirow{2}{*}{ILMT}                    & Test & 14.5 & 13.4 & 12.1 & 47.99 & 63.63 & 6.69 & 8.71 & 15.7 & 17.4 & 116.9 & 138.9 \\ \cline{2-13} 
                                         & Val  & 13.9 & 13   & 11.6 & 53.80 & 60.10 & 6.97 & 8.20 & 18.2 & 9.1  & 97.9  & 100.5 \\ \hline
\multirow{2}{*}{\sysname} & Test & 14.1 & 13.1 & 11.8 & 52.23 & 69.32 & 6.59 & 8.26 & 15.3 & 17.9 & 113.8 & 116.7 \\ \cline{2-13} 
                                         & Val  & 13.6 & 12.7 & 11.4 & 54.24 & 60.86 & 6.59 & 7.92 & 17.8 & 8.5  & 96.6  & 100   \\ \hline
RNN\_T                                   & Test-Banking & 14.2 & 13.3 & 12   & 66.93 & 68.23 & 9.26 & 9.92 & 28.8 & 7.3  & 105.9 & 100   \\ \hline
ILMT                                     & Test-Banking & 14.2 & 13.1 & 11.8 & 69.32 & 70.58 & 9.06 & 9.16 & 29.5 & 6.8  & 111.8 & 100   \\ \hline
\sysname                  & Test-Banking & 13.8 & 12.8 & 11.5 & 63.51 & 59.60 & 7.09 & 8.41 & 28.3 & 6.7  & 117.6 &  108.3       \\ \hline
\end{tabular}
}
\end{table*}

==> table3.tex <==
\begin{table*}[] 
\begin{tabular}{lllrrrrrrrrrrrl}
 &
   &
   &
  \multicolumn{1}{l}{WER} &
  \multicolumn{1}{l}{CER} &
  \multicolumn{1}{l}{PER} &
  \multicolumn{1}{l}{R-PER-all} &
  \multicolumn{1}{l}{R-CER-all} &
  \multicolumn{1}{l}{En-PER-all} &
  \multicolumn{1}{l}{En-CER-all} &
  \multicolumn{1}{l}{En-WER\_outdomain} &
  \multicolumn{1}{l}{En-WER\_outdomain\_eng} &
  \multicolumn{1}{l}{R-WER\_outdomain} &
  \multicolumn{1}{l}{R-WER\_outdomain\_eng} &
  R-WER\_outdomain\_eng \\
IXMT          & Blind-Test & All & 14.2 & 13.2 & 11.9 & 47.32142857          & 58.54800937 & 6.541116319          & 0.08553126628 & 15   & 17.1 & 121.5 & 122.2 &  \\
IXMT          & Test       & All & 13.7 & 12.8 & 11.4 & 53.88185654          & 60.43862451 & 7.045683046          & 0.08301624591 & 17.5 & 9.5  & 96.8  & 99.8  &  \\
IXMT(dropout) & Blind-Test & All & 14.1 & 13.1 & 11.8 & 0.546875             & 0.644028103 & 0.06614401363        & 0.08261783943 & 15.2 & 17.9 & 113.8 & 111.1 &  \\
IXMT(dropout) & Test       & All & 13.6 & 12.7 & 11.4 & \multicolumn{1}{l}{} & 61.73746407 & \multicolumn{1}{l}{} & 0.0785494491  & 17.7 & 8.5  & 97    & 100.2 & 
\end{tabular}
\caption{Ablation}
\label{tab:my-table}
\end{table*}

==> table3vinit.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{FFFFFF} 
Test &
  Split &
  Method &
  WER &
  CER &
  PER &
  \begin{tabular}[c]{@{}c@{}}Rare\\ PER\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Rare\\ CER\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Entity\\ PER\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Entity\\ CER\end{tabular} &

  \begin{tabular}[c]{@{}c@{}}Entity\\ WER\\OD\_Hi\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Entity\\ WER\\OD\_En\end{tabular} \\ \hline
 &
   &
  RNN-T &
  21.20 &
  19.20 &
  16.20 &
  71.80 &
  76.24 &
  21.39 &
  22.52 &
  33.20 &
  35.20 \\ \cline{3-12} 
 &
   &
  ILMT &
  21.30 &
  18.80 &
  17.10 &
  66.14 &
  \textbf{70.67} &
  21.54 &
  23.00 &
  33.20 &
  34.50 \\ \cline{3-12} 
 &
  \multirow{-3}{*}{Val} &
  \textbf{\sysnmae} &
  \textbf{20.50} &
  \textbf{18.00} &
  \textbf{16.30} &
  \textbf{67.13} &
  71.95 &
  \textbf{20.40} &
  \textbf{21.40} &
  \textbf{31.50} &
  \textbf{37.00} \\ \cline{2-12} 
 &
   &
  RNN-T &
  22.40 &
  20.00 &
  18.50 &
  70.88 &
  75.95 &
  24.53 &
  25.85 &
  37.70 &
  40.40 \\ \cline{3-12} 
 &
   &
  ILMT &
  \textbf{22.40} &
  19.50 &
  17.90 &
  67.14 &
  71.05 &
  24.58 &
  26.51 &
  38.60 &
  40.60 \\ \cline{3-12} 
\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Test-\\ \\ BANKING\end{tabular}} &
  \multirow{-3}{*}{Test} &
  \textbf{\sysname} &
  \textbf{21.50} &
  \textbf{18.70} &
  \textbf{17.10} &
  \textbf{67.44} &
  \textbf{71.77} &
  \textbf{22.34} &
  \textbf{23.44} &
  \textbf{37.00} &
  \textbf{38.70} \\ \hline
 &
   &
  RNN-T &
  18.70 &
  17.40 &
  15.90 &
  67.61 &
  73.90 &
  30.78 &
  34.23 &
  30.80 &
  60.30 \\ \cline{3-12} 
 &
   &
  ILMT &
  18.90 &
  17.40 &
  15.80 &
  63.78 &
  69.84 &
  28.46 &
  32.61 &
  30.70 &
  59.80 \\ \cline{3-12} 
 &
  \multirow{-3}{*}{Val} &
  \textbf{\sysname} &
  \textbf{17.80} &
  \textbf{16.10} &
  \textbf{14.60} &
  \textbf{58.39} &
  \textbf{63.73} &
  \textbf{28.52} &
  \textbf{31.60} &
  \textbf{29.40} &
  \textbf{58.30} \\ \cline{2-12} 
 &
   &
  RNN-T &
  18.40 &
  17.70 &
  16.10 &
  70.17 &
  76.68 &
  41.56 &
  45.25 &
  53.70 &
  38.30 \\ \cline{3-12} 
 &
   &
  ILMT &
  18.70 &
  17.60 &
  15.90 &
  65.75 &
  72.20 &
  37.85 &
  42.28 &
  54.30 &
  39.40 \\ \cline{3-12} 
\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Test-\\ INSURANCE\end{tabular}} &
  \multirow{-3}{*}{Test} &
  \textbf{\sysname} &
  \textbf{17.70} &
  \textbf{16.40} &
  \textbf{14.80} &
  \textbf{60.69} &
  \textbf{67.20} &
  \textbf{36.04} &
  \textbf{40.14} &
  \textbf{50.40} &
  \textbf{36.70} \\ \hline
 &
   &
  RNN-T &
  23.70 &
  21.60 &
  19.80 &
  72.44 &
  78.24 &
  49.21 &
  50.79 &
  40.90 &
  79.20 \\ \cline{3-12} 
 &
   &
  ILMT &
  23.40 &
  20.80 &
  18.90 &
  68.07 &
  74.62 &
  44.18 &
  46.26 &
  43.40 &
  81.70 \\ \cline{3-12} 
 &
  \multirow{-3}{*}{Val} &
  \textbf{\sysname} &
  \textbf{22.70} &
  \textbf{20.30} &
  \textbf{18.50} &
  \textbf{68.55} &
  \textbf{74.99} &
  \textbf{47.50} &
  \textbf{50.12} &
  \textbf{42.10} &
  \textbf{79.20} \\ \cline{2-12} 
 &
   &
  RNN-T &
  24.70 &
  22.40 &
  20.60 &
  76.74 &
  81.29 &
  46.77 &
  45.77 &
  50.40 &
  74.20 \\ \cline{3-12} 
 &
   &
  ILMT &
  24.50 &
  21.40 &
  19.70 &
  72.41 &
  77.52 &
  \textbf{39.11} &
  \textbf{38.15} &
  55.50 &
  69.10 \\ \cline{3-12} 
\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Test-\\ RETAIL\end{tabular}} &
  \multirow{-3}{*}{Test} &
  \textbf{\sysname} &
  \textbf{23.70} &
  \textbf{21.20} &
  \textbf{19.50} &
  \textbf{72.18} &
  \textbf{78.35} &
  45.41 &
  43.70 &
  \textbf{50.00} &
  \textbf{68.30} \\ \hline
 &
   &
  RNN-T &
  19.00 &
  18.80 &
  17.20 &
  72.07 &
  76.70 &
  17.43 &
  18.87 &
  19.90 &
  28.90 \\ \cline{3-12} 
 &
   &
  ILMT &
  19.20 &
  18.30 &
  16.60 &
  63.84 &
  70.21 &
  16.47 &
  18.32 &
  19.50 &
  24.40 \\ \cline{3-12} 
 &
  \multirow{-3}{*}{Val} &
  \textbf{\sysname} &
  \textbf{18.40} &
  \textbf{17.70} &
  \textbf{16.10} &
  \textbf{62.97} &
  \textbf{67.74} &
  \textbf{16.40} &
  \textbf{17.97} &
  \textbf{19.80} &
  \textbf{25.20} \\ \cline{2-12} 
 &
   &
  RNN-T &
  19.40 &
  18.60 &
  17.10 &
  68.27 &
  72.57 &
  30.17 &
  33.26 &
  19.90 &
  61.00 \\ \cline{3-12} 
 &
   &
  ILMT &
  19.30 &
  18.10 &
  16.40 &
  63.79 &
  68.97 &
  29.31 &
  33.23 &
  20.00 &
  57.70 \\ \cline{3-12} 
\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Test-\\ TELCO\end{tabular}} &
  \multirow{-3}{*}{Test} &
  \textbf{\sysname} &
  \textbf{18.60} &
  \textbf{17.50} &
  \textbf{16.00} &
  \textbf{64.27} &
  \textbf{68.59} &
  \textbf{29.33} &
  \textbf{32.50} &
  \textbf{19.00} &
  \textbf{62.40} \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table*}

==> tabledr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\scalebox{0.7}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Method &
\begin{tabular}[c]{@{}l@{}}Test\\ Data\end{tabular} &
  WER &
  CER &
  PER &
  \begin{tabular}[c]{@{}l@{}}Rare\\ PER\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Rare\\ CER\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Entity\\ PER\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Entity\\ PER\end{tabular} \\ \hline
RNN-T &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Test\\ Banking\end{tabular}} &
  22.40 &
  20.00 &
  18.50 &
  70.88 &
  75.95 &
  24.53 &
  24.53 \\ \cline{1-1} \cline{3-9} 
\sysname &
   &
  \textbf{21.50} &
  \textbf{18.70} &
  \textbf{17.10} &
  \textbf{67.44} &
  \textbf{71.77} &
  \textbf{22.34} &
  \textbf{22.34} \\ \cline{1-1} \cline{3-9} 
DR &
   &
  22.2 &
  19.9 &
  18.4 &
  70.82 &
  74.64 &
  23.81 &
  23.81 \\ \hline
RNN-T &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Test\\ Insurance\end{tabular}} &
  18.40 &
  17.70 &
  16.10 &
  70.17 &
  76.68 &
  41.56 &
  41.56 \\ \cline{1-1} \cline{3-9} 
\sysname &
   &
  \textbf{17.70} &
  \textbf{16.40} &
  \textbf{14.80} &
  \textbf{60.69} &
  \textbf{67.20} &
  \textbf{36.04} &
  \textbf{36.04} \\ \cline{1-1} \cline{3-9} 
  DR &
   &
  18.1 &
  17.7 &
  16 &
  69.12 &
  75.57 &
  40.31 &
  40.31 \\ \hline
RNN-T &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Test\\ Retail\end{tabular}} &
  24.70 &
  22.40 &
  20.60 &
  76.74 &
  81.29 &
  46.77 &
  46.77 \\ \cline{1-1} \cline{3-9} 
\sysname &
   &
  \textbf{23.70} &
  \textbf{21.20} &
  \textbf{19.50} &
  \textbf{72.18} &
  \textbf{78.35} &
  \textbf{45.41} &
  \textbf{45.41} \\ \cline{1-1} \cline{3-9} 
DR &
   &
  24.6 &
  22.1 &
  20.4 &
  76.02 &
  81.30 &
  46.43 &
  46.43 \\ \hline
RNN-T &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Test\\ Telco\end{tabular}} &
  19.40 &
  18.60 &
  17.10 &
  68.27 &
  72.57 &
  30.17 &
  30.17 \\ \cline{1-1} \cline{3-9} 
\sysname &
   &
  \textbf{18.60} &
  \textbf{17.50} &
  \textbf{16.00} &
  \textbf{64.27} &
  \textbf{68.59} &
  \textbf{29.33} &
  \textbf{29.33} \\ \cline{1-1} \cline{3-9} 
DR &
   &
  19.1 &
  18.2 &
  16.8 &
  70.52 &
  73.73 &
  27.98 &
  27.98 \\ \hline
\end{tabular}
}
\caption{}
\label{tab:my-table}
\end{table}
